Unlocking the Global Synergies in Low-Rank Adapters

Low-rank Adaption (LoRA) has been the de-facto parameter-efficient fine-tuning technique for large language models. We present HeteroLoRA, a light-weight search algorithm that leverages zero-cost proxies to allocate the limited LoRA trainable parameters across the model for better fine-tuned performance. In addition to the allocation for the standard LoRA-adapted models, we also demonstrate the efficacy of HeteroLoRA by performing the allocation in a more challenging search space that includes LoRA modules and LoRA-adapted shortcut connections. Experiments show that HeteroLoRA enables improvements in model performance given the same parameter budge. For example, on MRPC, we see an improvement of 1.6% in accuracy with similar training parameter budget. We will open-source our algorithm once the paper is accepted.

==> algorithms/heterolora_dynamic.tex <==
\begin{algorithm}[H]
\caption{Dynamic HeteroLoRA training}\label{alg: dynamic heterlora}
\small
\begin{algorithmic}[0]
\Require{$model$, $\mathcal{D}_\text{train}$, $\mathcal{D}_\text{val}$, 
$max\_epoch > 0$,\\
\Call{train}{model, train\_set},
\Call{validate}{model, validation\_set}, \\
$saliency\in\{\texttt{CONSTANT}, \texttt{SNIP},\texttt{SYNFLOW},\texttt{GRAD-NORM},\texttt{ALPHA-TEST}\}$, \Comment{saliency proxy to use} \\
$strategy\in\{\texttt{combined},\texttt{separated}\}$, \Comment{module ranking method, see \Cref{sec: dyrealloc result}} \\
$enable\_rate \in (0, 100]$, \Comment{percentage of LoRA and shortcut modules to be enabled} \\
\Call{heterolora\_search}{model, saliency, strategy, enable\_rate}, \Comment{see \Cref{alg: heterlora search}} \\
$search\_T > 0$. \Comment{number of HeteroLoRA search to perform in every epoch}}
\\
\State $subepoch \gets \left\lceil \frac{|\mathcal{D}_\text{train}|}{search\_T} \right\rceil$
\State $epoch \gets 0$
\While{$epoch<max\_epoch$} 
    \For{$i := 0$ to $search\_T-1$}
        \State \Call{heterolora\_search}{$model$, $saliency$, $strategy$, $enable\_rate$} \Comment{find a LoRA rank allocation}
        \State \Call{train}{$model$, $\mathcal{D}_\text{train}$[$i\times subepoch$ : $(i+1)\times subepoch$]} \Comment{train the $model$ on a fraction of the training set}
    \EndFor
    \State \Call{validate}{$model$, $\mathcal{D}_\text{val}$} \Comment{validate the $model$}
    \State $epoch \gets epoch + 1$
\EndWhile
\end{algorithmic}
\end{algorithm}

==> algorithms/heterolora_search.tex <==
\begin{algorithm}[H]
\caption{HeteroLoRA search}\label{alg: heterlora search}
\small
\begin{algorithmic}[0]
\Require{$model$, \Comment{model whose LoRA and shortcut modules are to be enabled/disabled}\\
$saliency\in\{\texttt{CONSTANT}, \texttt{SNIP},\texttt{SYNFLOW},\texttt{GRAD-NORM},\texttt{ALPHA-TEST}\}$, \Comment{saliency proxy to use} \\
$strategy\in\{\texttt{combined},\texttt{separated}\}$, \Comment{module ranking method, see \Cref{sec: dyrealloc result}} \\
$enable\_rate \in (0, 100]$, \Comment{percentage of LoRA and shortcut modules to be enabled} \\
\Call{get\_saliency}{model, saliency\_name}. \Comment{compute the saliencies of modules in the model}
}
\\
\State $scores \gets$ \Call{get\_saliency}{$model$, $saliency$} \Comment{compute saliency score for every LoRA and shortcut module in $model$}
\If{$strategy$ = \texttt{combined}} \Comment{LoRA and shortcut modules ranked together}
    \ForAll{$module$ in $model$}
        \If{$module$ in top $enable\_rate\%$ of $scores$}
            \State $module.disable$ $\gets \texttt{False}$ \Comment{enable the $module$}
        \Else
            \State $module.disable \gets \texttt{True}$ \Comment{disable the $module$}
        \EndIf
    \EndFor
\Else \Comment{LoRA and shortcut modules ranked separately}
    \State $scores_\text{LoRA} \gets scores$ of LoRA modules
    \State $scores_\text{shortcut} \gets scores$ of shortcut modules
    \ForAll{$module$ in $model$}
        \If{$module$ in top $enable\_rate\%$ of $scores_\text{LoRA}$ \textbf{or} $module$ in top $enable\_rate\%$ of $scores_\text{shortcut}$}
            \State $module.disable$ $\gets \texttt{False}$ \Comment{enable the $module$}
        \Else
            \State $module.disable \gets \texttt{True}$ \Comment{disable the $module$}
        \EndIf
    \EndFor
\EndIf
\end{algorithmic}
\end{algorithm}

==> algorithms/heterolora_static.tex <==
\begin{algorithm}[H]
\caption{Static HeteroLoRA training}\label{alg: static heterlora}
\small
\begin{algorithmic}[0]
\Require{$model$, $\mathcal{D}_\text{train}$, $\mathcal{D}_\text{val}$, 
$max\_epoch > 0$,\\
\Call{train}{model, train\_set},
\Call{validate}{model, validation\_set}, \\
$saliency\in\{\texttt{CONSTANT}, \texttt{SNIP},\texttt{SYNFLOW},\texttt{GRAD-NORM},\texttt{ALPHA-TEST}\}$, \Comment{saliency proxy to use} \\
$strategy\in\{\texttt{combined},\texttt{separated}\}$, \Comment{module ranking method, see \Cref{sec: dyrealloc result}} \\
$zc\_train\_limit > 0$, \Comment{number of training batches to use for the zero-cost training} \\
$enable\_rate \in (0, 100]$, \Comment{percentage of LoRA and shortcut modules to be enabled} \\
\Call{heterolora\_search}{model, saliency, strategy, enable\_rate}. \Comment{see \Cref{alg: heterlora search}} \\
}
\\
\If{$saliency$ = \texttt{ALPHA-TEST}}
    \State \Call{train}{$model$, $\mathcal{D}_\text{train}$[0:$zc\_train\_limit$]} \Comment{zero-cost training for $zc\_train\_limit$ batches}
\EndIf
\State \Call{heterolora\_search}{$model$, $saliency$, $strategy$, $enable\_rate$} \Comment{find a LoRA rank allocation}
\State $epoch \gets 0$
\While{$epoch<max\_epoch$} 
    \State \Call{train}{$model$, $\mathcal{D}_\text{train}$} \Comment{train the $model$}
    \State \Call{validate}{$model$, $\mathcal{D}_\text{val}$} \Comment{validate the $model$}
    \State $epoch \gets epoch + 1$
\EndWhile
\end{algorithmic}
\end{algorithm}

==> algorithms/lora_module.tex <==
\begin{algorithm}[H]
\caption{LoRA module methods}\label{alg:lora}
\begin{algorithmic}[0]
\Require{$r > 0$, $\alpha > 0$, $W \in \mathbb{R}^{d_\text{out}\times d_\text{in}}$, $A \in \mathbb{R}^{d_\text{r}\times d_\text{in}}$, $W \in \mathbb{R}^{d_\text{out}\times d_\text{r}}$, $\mathtt{merged} \in \mathbb{B}$}

\Function{forward}{$x$} \Comment{compute the LoRA-adapted linear transformation}
    \If{$\mathtt{merged}$}
        \State $res \gets W x$
    \Else
        \State $res \gets W x + \frac{\alpha}{r} B A x$
    \EndIf
    \State \Return $res$
\EndFunction

\Function{merge}{}
    \If{$\mathtt{merged}$}
        \State \Return
    \Else
        \State $W \gets W + \frac{\alpha}{r}BA$ \Comment{merge $\Delta W$ to the pre-trained weight $W$}
        \State $\mathtt{merged} \gets \texttt{True}$
    \EndIf
\EndFunction

\Function{unmerge}{}
    \If{$\mathtt{merged}$}
        \State $W \gets W - \frac{\alpha}{r}BA$ \Comment{split $\Delta W$ from the merged weight $W' = \Delta W + W$}
        \State $\mathtt{merged} \gets \texttt{False}$
    \Else
        \State \Return
    \EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}

==> outline.tex <==
\section{Introduction}

\subsection{Motivation}
Diagram: project mechanism

\subsection{Related works}

\subsection{Contribution}


\section{Preparation}

\subsection{Background theory}
\subsubsection{NLP}
\subsubsection{PLM}
\subsubsection{LoRA}
\subsubsection{Residual Network}
\subsubsection{NAS}

\subsection{Models and datasets}

\subsection{Starting point}

\subsection{Requirements analysis}

\subsection{Software engineering techniques}
\subsubsection{Development model}
\subsubsection{Tools, libraries, package manager, licensing}
\subsubsection{Hardware, version control, backup}


\section{Implementation}

\subsection{Testing??}

\subsection{Dataset preprocessing}
\subsubsection{Download, caching}
\subsubsection{Data loading}
\subsubsection{Tokenisation}

\subsection{Implementing LoRA}
\subsubsection{LoRA modules}
\subsubsection{LoRA configuration}
\subsubsection{LoRA-adapted models}

\subsection{Implementing dynamic-LoRA-reallocation training}
\subsubsection{LoRA module importance testing}
\subsubsection{Dynamic LoRA (and shortcut??) reallocation}

\subsection{Implementing shortcut architecture}
\subsubsection{Shortcut modules and configuration}
\subsubsection{Shortcut-adapted models}

\subsection{Training strategy}
\subsubsection{Loss function and metrics}
\subsubsection{Optimiser and weight decay (and learning rate scheduler??)}
\subsubsection{Checkpointing}
\subsubsection{Hyperparameter tuning}
\subsubsection{Network architecture search??}

\subsection{Repository overview}


\section{Evaluation}

\subsection{LoRA-adapted model performance analysis}
\subsubsection{R = 8 vs. other FT methods}
Table: method (full FT, adapters, bitfit, lora) vs. dataset (GLUE) vs. \# trainable parameters \& accuracy (+- stdev if necessary for baselines)

\subsubsection{Ablation: different R, different matrices}
Table: dataset (SST2, MRPC??) \& matrices vs. r (1,2,4,8,32) vs. accuracy

\subsection{Transferability analysis}
\subsubsection{}{Model transferability}
Table: model (RoBERTa, LLaMA??) \& method (FT/lora) vs. dataset (GLUE) vs. accuracy

\subsubsection{}{Dataset transferability}
Table: method (FT/lora) vs. dataset (Alpaca, SuperGLUE??) \& metric vs. result

\subsection{Dynamic reallocation training performance analysis}
\subsubsection{Manual reallocation vs. Zero-proxy reallocation vs. Dynamic reallocation}
Table: method (manual (first/mid/last), zero-proxy, dynamic) vs. dataset (Alpaca, SST2, MRPC??) \& metrics vs. result

\subsubsection{Turn-on frequency in dynamic reallocation}

Heatmap: dataset (Alpaca, SST2, MRPC??) per diagram; layer vs. matrix vs. frequency

\subsubsection{Dynamic reallocation ablation: different frequency N}
Table: dataset (Alpaca, SST2, MRPC??) vs. N per epoch (1, 2, 5, 10??) vs. median result +- stdev

OR Curve: dataset (Alpaca, SST2, MRPC??) per diagram; N per epoch (1, 2, 5, 10??) vs. median result +- quartiles

\subsection{Shortcut architecture analysis}
\subsubsection{Residual projections + LoRA \& Dense projections + LoRA}
Table: model (only lora, resnet lora, densenet lora) vs. dataset (Alpaca, SST2, MRPC??) vs. lora config, shortcut config \& result

\subsubsection{Dynamic reallocation on Dense shortcuts + LoRA??}
Turn-on frequency

Heatmap: rectangular of lora modules + square (lower triangle matrix) of dense shortcut modules

Vs. baselines

Table: method (full FT, lora, AutoPEFT, dynamic reallocated lora, FT dense shortcut, dynamic reallocated dense shortcuts and lora) vs. dataset (??) vs. \# trainable parameters \& result (+- stdev if necessary for baselines)

\subsection{Success criteria}


\section{Conclusions}

\subsection{Achievements}

\subsection{Lessons learned}

\subsection{Future work}


\section{Bibliography}

\section{Appendices}

\subsection{Additional implementation background??}

\subsection{Experiment setup}

\subsection{Hyperparameters}

\subsection{Additional results (reproduce literature results??)}


\section{Project Proposal}

==> sections/preparation.tex <==
\chapter{Preparation}

\section{Background theory}

This section provides concepts and theories essential to the project. In this section, I will introduce the Transformer attention architecture, followed by an overview of pre-trained language models. Next, I will discuss low-rank adaptation (LoRA) in detail, and describe previous achievements in incorporating shortcut connections to models.

\subsection{Transformer architecture}
\label{sec: transformer arch}

Transformer \citep{transformer} is a network architecture based on the attention mechanism. It has become the mainstream architecture of pre-trained language models \citep{llmsurvey}. The attention mechanism performs weighted aggregation on a collection of features to make sure the learning ``pays more attention'' to important features. It has revolutionised sequence modelling by enabling the modelling of element dependencies, irrespective of their distance in the sequence, thereby discerning which elements warrant greater or lesser attention.

\paragraph{Attention} An attention function takes a \textit{query} and a collection of \textit{key}-\textit{value} pairs. For each key-value pair, a weight is calculated and assigned to the value based on a compatibility function of the query and the key. Then, the values will be aggregated, usually by summation, according to their corresponding weights \citep{transformer}.

The Transformer architecture is based on a specific attention function called ``Scaled Dot-Product Attention'', described as:
$$\mathrm{Attention}(Q,K,V) = \mathrm{softmax}\left(\frac{Q^TK}{\sqrt{d_k}}\right) V$$
where $d_k$ is the dimension of queries and keys; $Q\in \mathbb{R}^{d_k\times M}$ represents the set of query (column) vectors of dimension $d_k$, with $M$ queries in total; $K\in \mathbb{R}^{d_k\times N}$ represents the set of key vectors of dimension $d_k$, with $N$ keys in total; $V\in \mathbb{R}^{d_k\times N}$ represents the set of value vectors of dimension $d_v$, corresponding to the key vectors; and the $\mathrm{softmax}$ function $\mathbf{f}(\mathbf{z})_i = \frac{e^{z_i}}{\sum_{j=1}^{|\mathbf{z}|} e^{z_j}}$ turns a set of logits into probabilities. The scaling $\frac{1}{\sqrt{d_k}}$ maintains the variance of the dot product and thus avoids the logits being pushed to regions of the softmax function with extremely small gradients \citep{transformer}.

\paragraph{Multi-head attention} The Transformer extends the single-attention to multi-head attention, in which the queries, keys and values are split into $h$ groups of vectors of dimension $d_k'$, $d_k'$ and $d_v'$ respectively, and then $h$ attention functions, or attention heads, are applied to the $h$ groups of vectors respectively. This can be described as:
\begin{align*}
    \mathrm{MultiHead}(Q,K,V) &= W^O\,\mathrm{Concat}(\mathrm{head}_1,...,\mathrm{head}_h) \\
    \text{where } \mathrm{head}_i &= \mathrm{Attention}(W_i^Q Q, W_i^K K, W_i^V V)
\end{align*}
where $W_i^Q\in \mathbb{R}^{d_k'\times d_k}$, $W_i^K\in \mathbb{R}^{d_k'\times d_k}$, and $W_i^V\in \mathbb{R}^{d_v'\times d_v}$ represent learnable linear projections of the $i$th attention head that transform the original queries $Q$, keys $K$ and values $V$ of dimension $d_k$ or $d_v$ into dimension $d_k'$ or $d_v'$; $\mathrm{Concat}$ denotes concatenating the $h$ outputs of the attention heads; and $W^O\in \mathbb{R}^{d_\mathrm{model} \times hd_v'}$ represents another learnable linear projection that transforms the concatenated output of dimension $hd_v'$ into the model's embedding dimension $d_\mathrm{model}$ (explained in below).

Specifically, the self-attention mechanism is used in encoder-only and decoder-only language models relevant to this project. In self-attention, $Q$, $K$ and $V$ are taken from the embedding of the same sequence, therefore having $d_k = d_v = d_\mathrm{model}$.

Multi-head attention allows different attention heads to be trained to focus on different parts of the sequence \citep{transformer}. In practice, $d_k' = d_v' = d_\mathrm{model} / h$ is employed to maintain the computational cost and allow layering with constant model embedding dimension.

 In order to preserve the auto-regressive property (only previously generated tokens should be considered when generating the next), an attention mask is employed to mask out (setting to $-\infty$) illegal values in the input to the softmax (e.g.\ tokens after the currently generating token are masked out because they should be ``generated in future'') \citep{transformer}.

\paragraph{Feed-forward network module} The Transformer also contains a fully connected feed-forward network (FFN) module, or a multi-layer perceptron (MLP) module, after the attention module, which performs two linear transformations with a ReLU activation (which might be changed into other activations in some models) in between:
$$\mathrm{FFN}(\mathbf{x}) = \max(\mathbf{0}, W_1\mathbf{x} + \mathbf{b_1})W_2 + \mathbf{b_2}$$
where $W_1, W_2$ are the weights of the two fully connected layers, $\mathbf{b_1}, \mathbf{b_2}$ are biases of the two fully connected layers, and the $\max$ function represents the ReLU activation.

\paragraph{Residual connection and layer normalisation} A residual connection \citep{resnet} is applied around each self-attention or FFN module, followed by layer normalisation \citep{layernorm}. The residual connection takes the input to a module and adds it back to the output of the module. Thus, each module's output becomes:
$$\mathrm{LayerNorm}(\mathbf{x} + \mathrm{Module}(\mathbf{x}))$$

The benefits of the residual connections are discussed in \Cref{sec: shortcut connections}. Layer normalisation normalises a hidden state vector by re-shifting and re-scaling according to the mean and the variance over the vector, and then performs an element-wise linear transformation with learnable gains $\mathbf{g}$ and biases $\mathbf{b}$, resulting in:
$$\mathbf{y} = \frac{\mathbf{x} - \mathbb{E}[\mathbf{x}]}{\sqrt{\mathbb{V}[\mathbf{x}]}} \otimes \mathbf{g} + \mathbf{b}$$
where $\otimes$ denotes element-wise product, $\mathbb{E}[\cdot]$ denotes the expectation, and $\mathbb{V}[\cdot]$ denotes the variance. Layer normalisation fixes the mean and the variance of the hidden state vector in the model layer and, therefore becomes invariant to per training-case feature shifting and scaling, and avoids undesirable ``covariate shifts'' that negatively impact the gradient of the following module \citep{layernorm}.

\paragraph{Tokenisation and embedding} Specifically in natural language processing (NLP), tokenisation is firstly performed on an input sentence, in which the sentence is split into units of text called tokens. Next, an embedding layer encodes the input tokens into feature vectors, or input embeddings, of the model embedding dimension $d_\mathrm{model}$. The input embeddings are then passed into layers of Transformer blocks, and finally, the output vectors are decoded back into tokens. The embedding layer needs to learn an effective mapping between the set tokens and the input embedding vectors of dimension $d_\mathrm{model}$.

\paragraph{Positional embedding} Furthermore, since the attention mechanism ignores the sequential order of tokens, \textit{positional embeddings} are added to the input embeddings at the start of the model or to the attention states in each layer. The positional embeddings are feature vectors representing the positional information at each position of the sentence. They are generated from \textit{positional encodings} and by another learnable embedding layer. The positional encodings can be $[0, 1, 2, ...,(t_{\mathrm{max}} - 1)]$ in a sequence of length $t_\mathrm{max}$ (\textit{absolute} positional encoding), or the relative distance from the current position to other positions like $[..., -2, -1, 0, 1, 2, ...]$ (\textit{relative} positional encoding). After the embedding operation, either or both absolute and relative positional embeddings can be added to the input embeddings or the attention states \citep{posembed}.

\paragraph{Language model head} In \textit{language modelling} tasks, the model generates a new token by predicting the probabilities of having each token given the input tokens. In order to convert the Transformer layers' output embedding vector of dimension $d_\mathrm{model}$ into a probability distribution over the set of possible tokens, a trainable linear transformation followed by a softmax function, referred to as the ``language model head'', is used. Similarly, in \textit{sequence classification} tasks, a language model head is trained to take the last embedding output of a sequence and predict probabilities over a set of classes.


\subsection{Pre-trained language model (PLM) and fine-tuning}
\label{sec: pretrain and finetune}

With the development of deep learning and Transformer architecture in the last decade, the number of model parameters has increased rapidly. In order to fully train the model parameters and avoid overfitting, much larger datasets are required for training. However, constructing large labelled datasets for NLP is extremely expensive in terms of annotation costs \citep{llmsurvey}.

On the other hand, constructing large-scale unlabelled corpora is relatively straightforward. By employing unsupervised or self-supervised tasks such as language modelling, denoising autoencoder, and contrastive learning, unlabelled text data can facilitate the learning of effective representations \citep{gpt2, llmsurvey}. These representations can then be leveraged for various "downstream" tasks in the future.

\textbf{Pre-trained language models} (PLM) leverage this kind of \textit{pre-training} scheme to extract representation from large unannotated corpora. Pre-training (a) allows the model to learn universal language representations and helps with downstream tasks, (b) offers improved model initialisation for subsequent transfer learning on the downstream task (discussed later), and (c) serves as a form of regularisation to prevent overfitting on a small dataset \citep{llmsurvey}.

After pre-training the large language model (LLM) on several pre-training tasks with challenging and substantial data, \textit{transfer learning} can be performed on the PLM, in which the knowledge from the source (pre-training) task is adapted to a target (downstream) task. To make transfer learning effective, several aspects need to be considered. First, different pre-training tasks will have different effects for different downstream tasks. While language modelling has become the most popular pre-training task for its generalisability to solve a wide range of NLP problems, choosing appropriate pre-training tasks (e.g.\ next sentence prediction) can further benefit certain downstream tasks (e.g.\ question answering and natural language inference). Second, the choice of the PLM architecture can influence its performance on the downstream task. Third, the data distribution of the downstream task is expected to be approximate to the pre-training task \citep{llmsurvey}.

Fine-tuning and feature extraction are two common approaches to model transfer learning \citep{bert, llmsurvey}. In feature extraction, the parameters of the PLM are frozen, and the model is regarded as a feature extractor. More complicated task-specific architectures are usually required by feature extraction.

On the other hand, \textbf{fine-tuning} trains the parameters of the PLM on the downstream dataset and is usually more general and convenient for various downstream tasks \citep{llmsurvey}. Since the PLM can capture effective language representations well, the downstream-task-specific layer (the language model head mentioned in the last subsection) can become very simple.


\subsection{Low-rank adaptation (LoRA)}

Despite the scalability of fine-tuning over different downstream tasks, conducting a full fine-tuning on an LLM is often parameter-inefficient: every downstream task requires a large set of its own tuned parameters \citep{llmsurvey}. Therefore, a series of special fine-tuning strategies referred to as \textit{parameter-efficient tuning} (PET) was studied to resolve the issue.

PET adapters introduce a small set of trainable parameters. These parameters of the adapter modules are trained on each downstream task while the pre-trained model parameters remain fixed. Switching between model versions of different downstream tasks only requires changing the tuned adapter modules.

\textbf{Low-rank adaptation} (LoRA) \citep{lora} is an adapter method that exploits the intrinsic low-rank structures in deep learning. The LoRA module is placed directly on top of pre-trained matrices and thus can be merged during inference to avoid extra inference latency.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/lora_overview.pdf}
    \caption{Overview of LoRA applied to a Transformer model. LoRA can be applied to each Transformer block. Taking a multi-head attention submodule in a block as an example, LoRA can be applied to linear projections transforming $Q$, $K$, $V$ and the concatenated output. For each LoRA module, the input is transformed by both a pre-trained weight $W$ and two low-rank matrices $A$ and $B$, whose results are added and returned.}
    \label{fig: lora}
\end{figure}

Mathematically, LoRA hypothesises that the updates $\Delta W$ to the pre-trained weights during fine-tuning have a low ``intrinsic rank''. Consequently, the update can be represented as the product of two rectangular low-rank decomposition matrices, yielding:
$$W_0 + \Delta W = W_0 + BA$$
where $W_0\in \mathbb{R}^{d\times k}$ denotes the pre-trained matrix, $\Delta W\in \mathbb{R}^{d\times k}$ denotes the update, and $B\in \mathbb{R}^{d\times r}$ and $A\in\mathbb{R}^{r\times k}$ with rank $r \ll \min(d,k)$ represents the low-rank decomposition matrices. By setting the LoRA rank $r$ to the rank of the pre-trained weight matrices, the expressiveness of full fine-tuning is roughly recovered by updating only the decomposition matrices. In other words, as $r$ increases, fine-tuning the LoRA-adapted model roughly converges to full fine-tuning on the original PLM \citep{lora}.

During fine-tuning, only the matrices $A$ and $B$ are unfrozen, yielding much less trainable parameters: $d\times r + r\times k = (d+k)\times r \ll d\times k$. 

To avoid shifts of the variance in the matrix product for a similar reason as in the Scaled Dot-Product Attention, a scaling factor $\frac{\alpha}{r}$ is introduced to $BA$, where $\alpha$ is a pre-defined constant acting as a scaling on the learning rate over the LoRA modules.

In order to keep $\Delta W = 0$ at the beginning of the fine-tuning, the decomposition matrix $A$ is initialised by random Gaussian, while matrix $B$ is initialised to zeros.

In practice, LoRA can be applied to the Transformer architecture on several linear transformations, including the linear projections $W_i^Q$, $W_i^K$, $W_i^V$ and $W^O$ in the attention module and the two fully-connected layers $W_1$ and $W_2$ in the FFN module. For simplicity and parameter efficiency, the multi-head projections $W_i^Q$, $W_i^K$, $W_i^V$ are treated as single matrices $W^Q, W^K, W^V \in \mathbb{R}^{d_\mathrm{model}\times d_\mathrm{model}}$, and only a subset of linear transformations are adapted to LoRA. %Further study of the effect of adopting different combinations of linear transformations is discussed in the ablation experiment.


\subsection{Shortcut connections}
\label{sec: shortcut connections}

The residual connections in the Transformer architecture, as well as other shortcut connection architectures, have been well-explored and obtained significant performance.

The residual connection has been employed by \textbf{ResNet} \citep{resnet} to image processing and achieved impressive results. The residual connection acts as an identity shortcut, taking the input to a function and adding it back to the function's output. 

The significance of the residual connection lies in addressing the optimisation difficulty as model depth increases. As depth grows, accuracy degradation occurs beyond a certain threshold. ResNet proposed that deep models may struggle to approximate identity mappings effectively using multiple non-linear layers. To address this, ResNet introduced residual connections, enabling the model to learn residual mappings more efficiently. By fitting a residual mapping $\mathcal{F}(\mathbf{x}) \triangleq \mathcal{H}(\mathbf{x}) - \mathbf{x}$ to achieve the desired mapping $\mathcal{H}(\mathbf{x})$, the model becomes easier to optimise \citep{resnet}.

Beyond the residual learning, shortcut connections have also been used to model certain kinds of \textit{inter-dependencies} between model blocks. In the \textbf{SENet} \citep{squeezeandexcitation}, a ``squeeze-and-excitation'' operation is introduced after a block of transformations (e.g.\ convolutions) to model channel dependencies explicitly. The operation first ``squeezes'' the global spatial information by averaging across the $C$ channels; then ``excites'' the vector of averages using two fully connected layers to capture the inter-dependencies with $\mathbf{s}\in \mathbb{R}^C$; and finally rescales the original channels according to $\mathbf{s}$. This kind of information flow aids the SENet in achieving significant improvement across models with various depths.

% Beyond the residual learning, shortcut connections have also been used to model certain kinds of \textit{inter-dependencies} between model blocks. In the \textbf{SENet} \citep{squeezeandexcitation}, a ``squeeze-and-excitation'' operation is introduced after a block of transformations (e.g.\ convolutions) to model channel dependencies explicitly. The squeeze-and-excitation operation works as a module that connects all input channels, extracting global information embeddings from them and performing feature recalibration back on the channels. The operation first ``squeezes'' the global spatial information by taking the average on each channel; then ``excites'' the vector of averages $\mathbf{z}\in \mathbb{R}^C$ to capture the inter-dependencies by two fully connected layers forming a bottleneck:
% $$\mathbf{s} = \mathrm{sigmoid}(W_2 \mathrm{ReLU}(W_1 \mathbf{z}))$$
% where $W_1 \in \mathbb{R}^{\frac{C}{r}\times C}$ and $W_2 \in \mathbb{R}^{C\times \frac{C}{r}}$ reduces the dimensionality by the ratio $r$, a trade-off between performance and computational cost; finally, similar to the attention mechanism, rescales the original channels according to $\mathbf{s}$. This kind of information flow aids the SENet in achieving significant improvement across models with various depths.

\textbf{DenseNet} \citep{densenet} offers an intuitive shortcut-adapted architecture. It divides a deep convolutional network into blocks based on feature map sizes. Within each block, the input to the current layer includes outputs from all preceding layers. Unlike ResNet's residual connections, DenseNet concatenates feature maps from previous layers rather than summing them, enhancing information flow. Consequently, DenseNet achieves the following: (a) forms a global state of "collective knowledge" accessible to any network layer; (b) promotes feature reuse, enhancing parameter efficiency; and (c) allows individual layers to receive additional supervision from the loss through shorter connections, addressing the vanishing-gradient problem and reinforcing feature propagation.

% \subsection{Automated PET}

% Numerous PET methods have achieved decent performances. However, deciding the optimal PET methods and PET configurations to use for a specific task is sophisticated and time-consuming. To this end, approaches have been proposed to automate the search process in PET.

% Neural architecture search (NAS) aims to find an optimal neural network architecture under certain constraints. Several previous works have applied NAS methods to automated PET searching. \textit{AutoPEFT} \citep{autopeft} has employed Bayesian optimisation \citep{bo} to search for Pareto-optimal configurations of models adapted to Serial Adapters \citep{serialadapter}, Parallel Adapters \citep{paralleladapter}, and prefix tuning \citep{prefixtuning}. \textit{S3PET} \citep{s3pet} has utilised DARTS \citep{darts}, a gradient-based NAS approach, to several PET methods. A framework conducting parameter pruning on LoRA and BitFit \citep{bitfit} has also been proposed \citep{nas4pet}. These studies have demonstrated the effectiveness of NAS in configuring a combination of PET methods.

% Specific methods for automating LoRA have also been studied. In \textit{DyLoRA} \citep{dylora}, training of LoRA modules employs a nested dropout which randomly selects a value $b$ and drops the ranks higher than $b$ in the decomposition matrices $A$ and $B$, therefore enforcing ordered representations in $A$ and $B$ and achieving the effect of training LoRA modules over a range of ranks $r$ simultaneously. Furthermore, in \textit{AdaLoRA} \citep{adalora}, the low-rank decomposition of the update matrix $\Delta W = BA$ is converted into an approximation of singular vector decomposition (SVD) $\Delta W = P\Lambda Q$ by applying regularisation terms to $P$ and $Q$ to enforce orthogonality. The singular values in $\Lambda$ are then pruned (i.e.\ set to zeros) in every training step according to their importance scores. The importance score employs the gradient-weight product of each parameter to estimate the sensitivity of loss to the parameter:
% $$I(w_{ij}) = \left|w_{ij} \cdot \nabla_{w_{ij}}\mathcal{L} \right|$$
% which then goes through a smoothing that considers the uncertainty of the importance score. These works have provided insights into designing the LoRA searches in this project.



\section{Models and datasets}

To assess LoRA's scalability and transferability across models, three pre-trained language models (PLMs) are utilized: Open Pre-trained Transformers (\textbf{OPT}) \citep{opt}, a family of decoder-only PLMs; Robustly optimized BERT approach (\textbf{RoBERTa}) \citep{roberta}, an enhanced variant of BERT models; and \textbf{Gemma} \citep{gemma}, a suite of models based on Google's Gemini models. Specifically, OPT-350M, RoBERTa-large, and Gemma-2B model versions are selected for evaluation, with their configurations provided in \Cref{tab: models}.

\input{tables/models}

Three categories of downstream tasks are employed: \textbf{sentiment analysis}, where the model needs to analyse the polarity of a sentence; \textbf{textual entailment}, where the model needs to determine the contextual relevance of input texts; and \textbf{causal language modelling}, where the model needs to predict the next token of an unfinished sentence. 

To align with the datasets utilised in the original works, nine datasets are selected for the three tasks, sourced from the GLUE benchmark \citep{glue}, SuperGLUE benchmark \citep{superglue}, and the Alpaca dataset employed in training the Stanford Alpaca model \citep{alpaca}, detailed in \Cref{tab: datasets}. Due to the lack of published test splits for most datasets, model performances are evaluated using the validation split as a common practice.

\input{tables/datasets}



\section{Starting point}

I have experience implementing machine learning algorithms using TensorFlow \citep{tensorflow}. However, my experience is limited to simple algorithms and I have no experience with PyTorch and Huggingface. I spent my initial weeks familiarising myself with the libraries.

My foundation knowledge of large language models (LLMs) and Transformer architecture was gained during the summer internship. I have experience in deploying LLMs on GPU servers but no experience in fine-tuning LLMs or PET methods. 

My basic concepts about parameter-efficient tuning (PET) and LoRA also came from the summer, but I was unfamiliar with the detailed mechanisms of LoRA and other PET methods. An open-sourced LoRA module implementation \citep{peft} is available, which has been referenced in the project and re-designed to accommodate my extension works including the LoRA allocation search and shortcut-adapted architectures.

I have basic knowledge of the theories of neural architecture search (NAS) but no experience of implementing a NAS or configuration search algorithm. I start with no knowledge of the theories of shortcut connections in neural networks.



\section{Requirements analysis}

\input{tables/req_analysis}


The requirements are derived from the Success Criteria of the Project Proposal, with additional components identified to support the aims of the extensions. \Cref{tab: req analysis} provides an overview of the requirements. Deliverables critical to achieving the core success criteria are marked \textcolor{red}{High}; those not strictly necessary but support a broader scope of exploration are marked \textcolor{BurntOrange}{Medium}; those not necessary but nice-to-have are marked \textcolor{Green}{Low}. The risk levels of deliverables represent the difficulty of the implementations. Components with \textcolor{Green}{Low} risk level have adequate open-sourced references; those with \textcolor{BurntOrange}{Medium} risk level have limited references; those with \textcolor{red}{High} risk level have no existing open-sourced implementation.



\section{Software engineering techniques}

\subsection{Development model}

This project adopts the Agile software development methodology since the research-oriented extensions may require iterative evaluations and re-designs. The Agile methodology breaks the development work into small increments accomplished by short sprints of development cycles as in \Cref{fig: agile}

\begin{figure}[b]
    \centering
    \includegraphics[width=\textwidth]{images/agile.pdf}
    \caption{Agile methodology development cycle}
    \label{fig: agile}
\end{figure}

In each Agile development cycle, an analysis of requirements and dependencies between components occurs. Subsequently, subsystems are designed by specifying APIs of object-oriented modules and creating flowcharts and data flow diagrams. In the implementation phase, documentation and code comments are added to enhance maintainability, and unit tests are performed to ensure correctness. Finally, evaluations and analyses are conducted, including comparisons with existing research results to ensure overall correctness.

The Agile cycle is iterated for the implementation of every LoRA-/shortcut-adapted model, every dataset, and every LoRA configuration search method. New findings that arose during the project would lead to extra explorations in the extensions.


\subsection{Tools, libraries, package manager and licenses}

Python is selected as the primary programming language of this project for its matured ecosystem of libraries and tools supporting machine learning and abundant open-sourced machine learning codebases. To handle deep learning works, \textbf{PyTorch} \citep{pytorch} is chosen for its flexibility and customisability in neural network and pipeline designing and GPU/CUDA supports. Meanwhile, \textbf{PyTorch Lightning} \citep{lightning}, a wrapper framework of PyTorch offering a lightweight training pipeline, is employed for its integrated functionality, high-level interfaces, and support of distributed parallel training. 

Following the \textit{Paper Checklist Guideline}\footnotemark[1] from the NeurIPS conference, this project uses PyTorch Lightning's function \texttt{seed\_everything} to set the seed for random generators in libraries to guarantee reproducibility.

\footnotetext[1]{NeurIPS 2022 Paper Checklist Guidelines: \url{https://neurips.cc/Conferences/2022/PaperInformation/PaperChecklist}}

For loading pre-trained language models and datasets, the \textbf{Huggingface} \citep{huggingface} platform is used. Huggingface provides a wide range of libraries including \texttt{tranformers} and \texttt{datasets} for open-sourced code, pre-trained model weights, and datasets.

The \textbf{Anaconda} package manager \citep{anaconda} is employed. It offers package dependency tracking, enabling easy reproduction of previous experiments over machines. 

This project has been released under Apache License 2.0 \citep{apache2.0}, allowing future researchers to build on my work. \Cref{tab: licenses} lists important third-party libraries used in this project, their functionality and OSI-approved \citep{osi} licenses.

\input{tables/licences}


\subsection{Hardware setup and version control}

I use my laptop for code and dissertation writing. The laptop is a ThinkPad X1 Carbon Gen 8 (1.10 GHz Intel Core i7, 16 GB RAM, Windows 10, Intel UHD Graphics 8195 MB). Experiments are run on a server with 4 NVIDIA QUADRO RTX 8000 GPUs provided by the department, as well as the HPC cluster with servers of 3 NVIDIA A100 40 GB RAM Tensor Core GPUs, 2 AMD EPYC 7742 (Rome) 2.25 GHz 64-core processors, and 512 GB DDR4-3200 RAM provided by Sulis.

I use Git for version control, with a remote GitHub repository as a backup that is synchronised with the local repository regularly. Experiment results are backed up in Google Drive. LaTeX and the Overleaf platform are used for dissertation writing and backup. 


==> sections/related.tex <==
\section{Related Works}

\subsection{Low-Rank Adaptation}

Despite the scalability of fine-tuning over different downstream tasks, conducting a full fine-tuning on an LLM is often parameter-inefficient: every downstream task requires a large set of its own tuned parameters \citep{llmsurvey}. Therefore, a series of special fine-tuning strategies referred to as \textit{parameter-efficient tuning} (PET) was studied to resolve the issue.

PET adapters introduce a small set of trainable parameters. These parameters of the adapter modules are trained on each downstream task while the pre-trained model parameters remain fixed. Switching between model versions of different downstream tasks only requires changing the tuned adapter modules.

\textbf{Low-rank adaptation} (LoRA) \citep{lora} is an adapter method that exploits the intrinsic low-rank structures in deep learning. The LoRA module is placed directly on top of pre-trained matrices and thus can be merged during inference to avoid extra inference latency.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/lora_overview.pdf}
    \caption{Overview of LoRA applied to a Transformer model. LoRA can be applied to each Transformer block. Taking a multi-head attention submodule in a block as an example, LoRA can be applied to linear projections transforming $Q$, $K$, $V$ and the concatenated output. For each LoRA module, the input is transformed by both a pre-trained weight $W$ and two low-rank matrices $A$ and $B$, whose results are added and returned.}
    \label{fig: lora}
\end{figure}

Mathematically, LoRA hypothesises that the updates $\Delta W$ to the pre-trained weights during fine-tuning have a low ``intrinsic rank''. Consequently, the update can be represented as the product of two rectangular low-rank decomposition matrices, yielding:
$$W_0 + \Delta W = W_0 + BA$$
where $W_0\in \mathbb{R}^{d\times k}$ denotes the pre-trained matrix, $\Delta W\in \mathbb{R}^{d\times k}$ denotes the update, and $B\in \mathbb{R}^{d\times r}$ and $A\in\mathbb{R}^{r\times k}$ with rank $r \ll \min(d,k)$ represents the low-rank decomposition matrices. By setting the LoRA rank $r$ to the rank of the pre-trained weight matrices, the expressiveness of full fine-tuning is roughly recovered by updating only the decomposition matrices. In other words, as $r$ increases, fine-tuning the LoRA-adapted model roughly converges to full fine-tuning on the original PLM \citep{lora}.

During fine-tuning, only the matrices $A$ and $B$ are unfrozen, yielding much less trainable parameters: $d\times r + r\times k = (d+k)\times r \ll d\times k$. 

To avoid shifts of the variance in the matrix product for a similar reason as in the Scaled Dot-Product Attention, a scaling factor $\frac{\alpha}{r}$ is introduced to $BA$, where $\alpha$ is a pre-defined constant acting as a scaling on the learning rate over the LoRA modules.

In order to keep $\Delta W = 0$ at the beginning of the fine-tuning, the decomposition matrix $A$ is initialised by random Gaussian, while matrix $B$ is initialised to zeros.

In practice, LoRA can be applied to the Transformer architecture on several linear transformations, including the linear projections $W_i^Q$, $W_i^K$, $W_i^V$ and $W^O$ in the attention module and the two fully-connected layers $W_1$ and $W_2$ in the FFN module. For simplicity and parameter efficiency, the multi-head projections $W_i^Q$, $W_i^K$, $W_i^V$ are treated as single matrices $W^Q, W^K, W^V \in \mathbb{R}^{d_\mathrm{model}\times d_\mathrm{model}}$, and only a subset of linear transformations are adapted to LoRA.



\subsection{Shortcut Connections}
\label{sec: shortcut connections}

The residual connections in the Transformer architecture, as well as other shortcut connection architectures, have been well-explored and obtained significant performance.

The residual connection has been employed by \textbf{ResNet} \citep{resnet} to image processing and achieved impressive results. The residual connection acts as an identity shortcut, taking the input to a function and adding it back to the function's output. 

The significance of the residual connection lies in addressing the optimisation difficulty as model depth increases. As depth grows, accuracy degradation occurs beyond a certain threshold. ResNet proposed that deep models may struggle to approximate identity mappings effectively using multiple non-linear layers. To address this, ResNet introduced residual connections, enabling the model to learn residual mappings more efficiently. By fitting a residual mapping $\mathcal{F}(\mathbf{x}) \triangleq \mathcal{H}(\mathbf{x}) - \mathbf{x}$ to achieve the desired mapping $\mathcal{H}(\mathbf{x})$, the model becomes easier to optimise \citep{resnet}.

Beyond the residual learning, shortcut connections have also been used to model certain kinds of \textit{inter-dependencies} between model blocks. In the \textbf{SENet} \citep{squeezeandexcitation}, a ``squeeze-and-excitation'' operation is introduced after a block of transformations (e.g.\ convolutions) to model channel dependencies explicitly. The operation first ``squeezes'' the global spatial information by averaging across the $C$ channels; then ``excites'' the vector of averages using two fully connected layers to capture the inter-dependencies with $\mathbf{s}\in \mathbb{R}^C$; and finally rescales the original channels according to $\mathbf{s}$. This kind of information flow aids the SENet in achieving significant improvement across models with various depths.

% Beyond the residual learning, shortcut connections have also been used to model certain kinds of \textit{inter-dependencies} between model blocks. In the \textbf{SENet} \citep{squeezeandexcitation}, a ``squeeze-and-excitation'' operation is introduced after a block of transformations (e.g.\ convolutions) to model channel dependencies explicitly. The squeeze-and-excitation operation works as a module that connects all input channels, extracting global information embeddings from them and performing feature recalibration back on the channels. The operation first ``squeezes'' the global spatial information by taking the average on each channel; then ``excites'' the vector of averages $\mathbf{z}\in \mathbb{R}^C$ to capture the inter-dependencies by two fully connected layers forming a bottleneck:
% $$\mathbf{s} = \mathrm{sigmoid}(W_2 \mathrm{ReLU}(W_1 \mathbf{z}))$$
% where $W_1 \in \mathbb{R}^{\frac{C}{r}\times C}$ and $W_2 \in \mathbb{R}^{C\times \frac{C}{r}}$ reduces the dimensionality by the ratio $r$, a trade-off between performance and computational cost; finally, similar to the attention mechanism, rescales the original channels according to $\mathbf{s}$. This kind of information flow aids the SENet in achieving significant improvement across models with various depths.

\textbf{DenseNet} \citep{densenet} offers an intuitive shortcut-adapted architecture. It divides a deep convolutional network into blocks based on feature map sizes. Within each block, the input to the current layer includes outputs from all preceding layers. Unlike ResNet's residual connections, DenseNet concatenates feature maps from previous layers rather than summing them, enhancing information flow. Consequently, DenseNet achieves the following: (a) forms a global state of "collective knowledge" accessible to any network layer; (b) promotes feature reuse, enhancing parameter efficiency; and (c) allows individual layers to receive additional supervision from the loss through shorter connections, addressing the vanishing-gradient problem and reinforcing feature propagation.


\subsection{Configuration search in PET}

Numerous PET methods have shown significant performance improvements. However, determining the most suitable methods and configurations for a given task can be complex and time-consuming. To address this challenge, various automated approaches to PET search have been proposed.

Neural Architecture Search (NAS) attempts to discover an optimal neural network architecture within predefined constraints. Prior research has explored applying NAS methods to automate the search for Parameter-Efficient Tuning (PET) strategies. For instance, \textit{AutoPEFT} \citep{autopeft} utilised Bayesian optimisation \citep{bo} to identify Pareto-optimal configurations for models adapted to Serial Adapters \citep{serialadapter}, Parallel Adapters \citep{paralleladapter}, and prefix tuning \citep{prefixtuning}. Another approach, \textit{S3PET} \citep{s3pet}, employed DARTS \citep{darts}, a gradient-based NAS technique, across various PET methods. Additionally, a framework integrating parameter pruning into LoRA and BitFit \citep{bitfit} was proposed \citep{nas4pet}.

Furthermore, several methods have emerged to enhance the LoRA algorithm for automatic selection of an optimal rank. In \textit{DyLoRA} \citep{dylora}, nested dropout is employed to enforce ordered representations in matrices $A$ and $B$, allowing simultaneous training of LoRA modules across a range of ranks $r$. This enables seamless switching between different rank configurations without the need for re-training. In contrast, \textit{AdaLoRA} \citep{adalora} modifies the low-rank decomposition of the update matrix $\Delta W = BA$ into an approximation of singular value decomposition (SVD) $\Delta W = P\Lambda Q$, achieved by applying regularisation terms to matrices $P$ and $Q$ to enforce orthogonality. Subsequently, singular values in matrix $\Lambda$ are pruned in each training step based on their importance scores, derived from the gradient-weight product of each parameter relative to the loss function.

However, these methods either necessitate computationally intensive full NAS or entail additional trainable parameters for the configuration search, while being confined to the existing architecture search space. \Cref{tab: feature cmp} provides a summary of the distinctions between HeteroLoRA and previous approaches.

\input{tables/feature_cmp}


==> tables/datasets.tex <==
\begin{table}[t!]
    \caption{Nine datasets selected for the project. The size of the training set and the validation set are reported. \textsuperscript{*}The Alpaca dataset is manually split into a training and a validation set by a ratio of 9 to 1 in this project.}
    \label{tab: datasets}
    \centering
    \small
    \begin{tabular}{>{\centering\arraybackslash}m{0.1\linewidth}>{\centering\arraybackslash}m{0.09\linewidth}>{\centering\arraybackslash}m{0.1\linewidth}>{\raggedright\arraybackslash}m{0.6\linewidth}}
    \toprule
    \textbf{Dataset} &
      \textbf{\#Train} &
      \textbf{\#Val} &
      \textbf{Description} \\
    \midrule
    SST-2 &
      67.3K &
      872 &
      A sentiment analysis task consists of sentences from movie reviews. The task is to predict the two-way sentiment (\textit{positive}/\textit{negative}) of a given sentence. \\
    \midrule
    MNLI &
      393K &
      19.7K &
      Given a premise and a hypothesis sentence, the task is to predict whether the premise entails or contradicts the hypothesis, or neither (neutral). \\
    \midrule
    MRPC &
      3.67K &
      408 &
      A corpus of sentence pairs extracted from online news sources with annotations for whether the sentences are semantically equivalent. \\
    \midrule
    QQP &
      364K &
      40.4K &
      A collection of question pairs from the community question-answering website Quora with annotations for whether the questions are semantically equivalent. \\
    \midrule
    RTE &
      2.49K &
      277 &
      A textual entailment task consists of data coming from a series of annual textual entailment challenges. \\ 
    \midrule
    BoolQ &
      9.43K &
      3.27K &
      A question-answering task with examples consisting of short passages and yes/no questions about the passages. \\
    \midrule
    CB &
      250 &
      56 &
      A textual entailment task with a corpus of short texts where at least one sentence contains an embedded clause. \\ 
    \midrule
    COPA &
      400 &
      100 &
      A causal reasoning task in which the model is given a premise sentence and must determine either the cause or effect of the premise from two possible choices. \\
    \midrule
    Alpaca &
      52K\textsuperscript{*} &
       &
      A dataset for language modelling generated by OpenAI's \texttt{text-davinci-003} engine based on the Self-Instruct framework \citep{selfinstruct}. \\
    \bottomrule
\end{tabular}
\end{table}

==> tables/dyrealloc_totalfreq.tex <==
\begin{table*}
    \caption{Frequency that LoRA modules were enabled throughout the dynamic HeteroLoRA training under three setups: separated allocation with $r=8$ or $r=32$, combined allocation with $r=8$, and combined allocation with $r=32$.}
    \label{tab:dyrealloc_totalfreq}
    \centering
    \begin{tabular}{c|c|c|c}
    \toprule
    Method & Separated Alloc           & Combined Alloc $r=8$ & Combined Alloc $r=32$ \\
    \midrule
    MRPC   & \multirow{3}{*}{$33.33\%$} & $61.49\%_{\pm 3.64\%}$ & $62.16\%_{\pm 0.22\%}$  \\
    RTE    &                           & $50.42\%_{\pm 2.51\%}$ & $51.48\%_{\pm 1.08\%}$   \\
    SST-2  &                           & $56.94\%_{\pm 1.35\%}$ & $59.94\%_{\pm 1.61\%}$                    \\
    % Alpaca &                           & $59.16\%_{\pm 1.62\%}$ & $61.06\%_{\pm 2.74\%}$                    \\
    \bottomrule
    \end{tabular}
\end{table*}

==> tables/feature_cmp.tex <==
\begin{table*}
    \caption{Comparison between HeteroLoRA and previous works over features including (a) single-shot NAS, where the search is accomplished in a single training run; (b) fixed GPU memory usage, where the searching process does not require more trainable parameters than the target parameter limitation; and (c) shortcut-enabled, where the search considers shortcut connections.}
    \label{tab: feature cmp}
    \centering
    \begin{tabular}{c|ccc}
    \toprule
    Features & \begin{tabular}[c]{@{}c@{}}Single-shot NAS\end{tabular} & \begin{tabular}[c]{@{}c@{}}Fixed GPU Memory Usage\end{tabular}& \begin{tabular}[c]{@{}c@{}}Shortcut-enabled\end{tabular} \\
    \midrule
    AutoPEFT \citep{autopeft}   &                            \ding{55}&                            \ding{51}&                           \ding{51}\\
    S3PET \citep{s3pet}       &                            \ding{51}&                            \ding{55}&                           \ding{55}\\
    NAS for PET \citep{nas4pet} &                            \ding{55}&                            \ding{55}&                           \ding{55}\\
    DyLoRA \citep{dylora}     &                            \ding{51}&                            \ding{55}&                           \ding{55}\\
    AdaLoRA \citep{adalora}    &                            \ding{51}&                            \ding{51}&                           \ding{55}\\
    HeteroLoRA  &                            \ding{51}&                            \ding{51}&                          
    \ding{51} \\
    \bottomrule
    \end{tabular}
\end{table*}

==> tables/licences.tex <==
\begin{table}
    \caption{A list of third-party libraries used in the project.}
    \label{tab: licenses}
    \centering
    \small
    \begin{tabular}{ccc}
    \toprule
    \textbf{Library} & \textbf{Usage} & \textbf{License} \\
    \midrule
    \texttt{torch} & Train and test neural networks & BSD License \\
    \texttt{pytorch\_lightning} & High-level interface for training & Apache License 2.0 \\
    \texttt{torchmetrics} & Metrics computing evaluation & Apache License 2.0 \\
    \texttt{numpy} & Manipulate multi-dimensional arrays & MIT License \\
    \texttt{transformers} & Huggingface library for PLMs & Apache License 2.0 \\
    \texttt{datasets} & Huggingface library for datasets & Apache License 2.0 \\
    \texttt{matplotlib} & Plot statistical diagrams & PSF License \\
    \texttt{seaborn} & Plot statistical diagrams & BSD License \\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/lora_abla_proj1.tex <==
\begin{table*}
    \caption{Performance of LoRA applied to different combinations of linear projections in the attention submodule under the same numbers of trainable parameters. Adapting $W^V$ and $(W^Q, W^V)$ perform the best.}
    \label{tab:lora_abla_proj1}
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|ccccccc}
    \toprule
    Projections & $W^Q$ & $W^K$ & $W^V$                           & $W^O$                & $W^Q, W^K$ & $W^Q, W^V$ & \begin{tabular}[c]{@{}c@{}} $W^Q, W^K,$ \\ $W^V, W^O$ \end{tabular} \\
    Rank $r$ & 8 & 8 & 8 & 8 & 4 & 4 & 2  \\
    % \midrule
    \midrule
    MRPC (acc) & $80.2{\pm 1.6}$  & $80.3{\pm 0.5}$ & $\mathbf{84.3{\pm 1.3}}$ & $83.2{\pm 0.1} $ & $81.6{\pm 1.1}$ & $\mathbf{84.1{\pm 1.1}}$ & $83.3{\pm 1.8}$ \\    
    \bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/lora_abla_proj2.tex <==
\begin{table*}
    \caption{Comparison of LoRA applied to attention linear projections, FFN linear projections, and both. Due to the larger feed-forward network module dimension, adapting FFN projections $W_1$ or $W_2$ costs more trainable parameters than the attention projections.}
    \label{tab:lora_abla_proj2}
    \centering
    % \resizebox{\textwidth}{!}{%
    \begin{tabular}{>{\centering\arraybackslash}m{0.16\linewidth}|>{\centering\arraybackslash}m{0.14\linewidth}|>{\centering\arraybackslash}m{0.1\linewidth}>{\centering\arraybackslash}m{0.1\linewidth}>{\centering\arraybackslash}m{0.14\linewidth}|>{\centering\arraybackslash}m{0.2\linewidth}}
    \toprule
    Projections & $W^Q, W^V$ & $W_1$ & $W_2$ & $W_1, W_2$ & $W^Q, W^V, W_1, W_2$ \\
    Rank $r$       & 4  & 8     & 8     & 4          & 2 \\
    % \midrule
    \# Trainable   & 394K & \multicolumn{3}{c|}{984K}                       & 689K \\
    \midrule
    MRPC (acc) & $\mathbf{84.1{\pm 1.1}}$ & $83.3{\pm 0.6}$ & $82.3{\pm 1.2}$ & $84.0{\pm 0.9}$ & $83.5{\pm 0.5}$ \\
    \bottomrule
    \end{tabular}
    % }
\end{table*}

==> tables/lora_abla_r.tex <==
\begin{table}[b]
    \caption{Performance of LoRA with different ranks $r$. LoRA is applied to the query and value projections. Surprisingly, performance ``saturates'' at a very small rank.}
    \label{tab:lora_abla_r}
    \centering
    \begin{tabular}{c|ccccc}
    \toprule
    LoRA rank & $r=1$       & $r=2$       & $r=4$       & $r=8$       & $r=32$      \\
    \midrule
    MRPC      & $83.3/80.7$ & $83.1/79.4$ & $84.1/81.0$ & $83.9/80.7$ & $83.9/80.5$ \\
    RTE       & $67.6$      & $73.4$      & $71.5$      & $71.1$      & $73.1$      \\
    SST2      & $93.5$      & $93.7$      & $93.9$      & $93.5$      & $93.9$      \\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/lora_datasets.tex <==
\begin{table*}
    \caption{LoRA performances compared to full fine-tuning (Full FT) on OPT-350M model. Accuracy and F1 score are reported for MRPC, QQP and CB; perplexity is reported for Alpaca; overall (matches and mismatches) accuracy is reported for MNLI; and accuracy is reported for other tasks. Except for the perplexity for Alpaca, higher is better for all metrics. Datasets marked * are extensions.}
    \label{tab:lora_datasets}
    \centering
    \begin{tabularx}{0.97\linewidth}{c|cccc}
        \toprule
        \textbf{Method} & \textbf{MNLI} & \textbf{MRPC}\textsubscript{ACC/F1} & \textbf{QQP}\textsubscript{ACC/F1} & \textbf{RTE} \\
        \midrule
        Full FT & $83.9\pm0.1$ & $82.6\pm0.9/79.0\pm1.5$ & $90.3\pm0.1/89.7\pm0.2$ & $72.3\pm1.5$ \\
        LoRA & $83.5\pm0.1$ & $84.1\pm1.1/80.7\pm1.2$ & $88.5\pm0.2/87.8\pm0.2$ & $73.0\pm1.6$ \\
        \bottomrule
    \end{tabularx}
    \begin{tabularx}{0.97\linewidth}{c|ccccc}
        \toprule
        \textbf{Method} & \textbf{SST-2} & \textbf{Alpaca}\textsuperscript{*}\textsubscript{PPL} & \textbf{BoolQ}\textsuperscript{*} & \textbf{CB}\textsuperscript{*}\textsubscript{ACC/F1} & \textbf{COPA}\textsuperscript{*} \\
        \midrule
        Full FT & $93.5\pm0.5$ & $6.21\pm0.01$ & $76.2\pm0.5$ & $82.1\pm4.4/70.5\pm9.7$ & $57.0\pm1.6$ \\
        LoRA & $93.4\pm0.5$ & $6.64\pm0.01$ & $75.8\pm0.5$ & $82.1\pm4.9/71.1\pm6.4$ & $57.0\pm1.5$ \\
        \bottomrule
    \end{tabularx}
\end{table*}

==> tables/lora_models.tex <==
\begin{table*}
    \caption{LoRA and full fine-tuning (FT) accuracy on GLUE datasets with three models. The number of trainable parameters for each fine-tuning method and model is demonstrated. For Gemma, full fine-tuning is not conducted due to the high memory requirement. The difference between LoRA and full fine-tuning performance is reported. The average accuracy weighted by dataset sizes is also reported. Results of models marked \textsuperscript{$\dagger$} are from prior works.}
    \label{tab:lora_models}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|r|cccccc}
    \toprule
    \multicolumn{1}{c|}{\textbf{Model}} & \multicolumn{1}{c|}{\textbf{\#Trainable}} & \textbf{MNLI}   & \textbf{MRPC}        & \textbf{QQP}         & \textbf{RTE}    & \textbf{SST2}   & \textbf{Avg\textsubscript{(acc)}}   \\
    \midrule
    OPT FT & $331.2$M & 83.9 & 82.6 & 90.3 & 72.3 & 93.5 & 87.5 \\
    OPT LoRA    & $0.8$M   & 83.5\textcolor{Red}{(-0.4)}& 84.1\textcolor{Green}{(+1.5)} & 88.5\textcolor{Red}{(-1.8)} & 73.0\textcolor{Green}{(+0.7)} & 93.4\textcolor{Red}{(-0.1)} & 86.5\textcolor{Red}{(-1.0)} \\
    \midrule
    RoB FT            & $355.0$M                            & 89.0 & 90.2 & 91.6 & 85.6 & 96.0 & 90.7 \\
    RoB LoRA               & $0.8$M                              & 89.9\textcolor{Green}{(+0.9)} & 90.2\textcolor{Green}{(+0.0)} & 90.9\textcolor{Red}{(-0.7)} & 87.1\textcolor{Green}{(+1.5)} & 95.6\textcolor{Red}{(-0.4)} & 90.8\textcolor{Green}{(+0.1)} \\
    \midrule
    RoB FT\textsuperscript{$\dagger$} & $355.0$M & 90.2 & 90.9 & 92.2 & 86.6 & 96.4 & 91.6 \\
    RoB LoRA\textsuperscript{$\dagger$} & $0.8$M & 90.6\textcolor{Green}{(+0.4)} & 90.9\textcolor{Green}{(+0.0)} & 91.6\textcolor{Red}{(-0.6)} & 87.4\textcolor{Green}{(+0.8)} & 96.2\textcolor{Red}{(-0.2)} & 91.5\textcolor{Red}{(-0.1)} \\
    \midrule
    Gemma LoRA  & $0.9$M   & 89.7 & 86.8 & 90.8 & 86.7 & 96.8 & 90.7 \\
    \bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/models.tex <==
\begin{table}
    \caption{Three models chosen for the project. The number of model parameters (\#Parameters), the number of layers (\#L), the number of attention heads (\#H), and the embedding size ($d_\mathrm{model}$) are reported. ``M'' denotes million and ``B'' denotes billion.}
    \label{tab: models}
    \centering
    \begin{tabular}{ccccc}
    \toprule
    \textbf{Model} & \textbf{\#Parameters} & \textbf{\#L} & \textbf{\#H} & \textbf{$d_\mathrm{model}$} \\
    \midrule
    OPT-350M      & $350$M   & $24$ & $16$ & $1024$ \\
    RoBERTa-large & $355$M   & $24$ & $16$ & $1024$ \\
    Gemma-2B      & $2.51$B & $18$ & $8$  & $2048$ \\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/r_search_avg.tex <==
\begin{table}
    \caption{Performance of LoRA applied to different combinations of linear projections in the attention submodule under the same numbers of trainable parameters. Adapting $W^K$ and $(W^Q, W^V)$ perform the best.}
    \label{tab:r-search-avg}
    \centering
    \begin{tabular}{c|ccc}
    \toprule
    \# Trainable               & 0.6M & 2.3M & 9.8M \\
    \midrule
    LoRA-only                  & 92.3 & 92.1 & 91.9 \\
    Shortcut + LoRA            & 92.3 & 92.6 & 92.7 \\
    Shortcut + LoRA with $r=2$ & 92.3 & 92.4 & 92.5 \\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/repo_overview.tex <==
\begin{figure}[H]
\setlength{\DTbaselineskip}{15pt}
\centering
\small
\dirtree{%
.1 .
.2 src/ \DTcomment{Code directory\: \bf 11499 lines}.
.3 actions/ \DTcomment{Machine learning pipelines\: \bf 513 lines}.
.4 train.py \DTcomment{Training pipeline\: \bf 158 lines}.
.4 test.py \DTcomment{Testing pipeline\: \bf 66 lines}.
.4 train\_dyrealloc.py \DTcomment{Dynamic LoRA-searching training pipeline\: \bf 206 lines}.
.4 pretrain\_alloc.py \DTcomment{Static LoRA allocation search pipeline\: \bf 79 lines}.
.3 dataset/ \DTcomment{Dataset preprocessing modules\: \bf 1320 lines}.
.3 \sethlcolor{Apricot}\hl{importance\_testing/} \DTcomment{Compute saliency heuristics statically\: \bf 855 lines}.
.3 loading/ \DTcomment{Set-up functions\: \bf 786 lines}.
.4 argparser\_ags.py \DTcomment{Specify and parse CLI argument\: \bf 429 lines}.
.4 config\_load.py \DTcomment{TOML configuration loader\: \bf 84 lines}.
.4 model\_loader.py \DTcomment{Load pre-trained model loader\: \bf 180 lines}.
.4 setup\_folders.py \DTcomment{Set up experiment log folder\: \bf 16 lines}.
.4 setup\_model\_and\_dataset.py \DTcomment{Preprocess dataset and prepare model\: \bf 54 lines}.
.4 tokenizer\_loader.py \DTcomment{Load pre-trained tokenizer\: \bf 23 lines}.
.3 \sethlcolor{Apricot}\hl{lora/} \DTcomment{LoRA module and configuration parser\: \bf 318 lines}.
.3 \sethlcolor{Salmon}\hl{models/} \DTcomment{LoRA-adapted and shortcut-adapted models\: \bf 4721 lines}.
.3 pl\_callbacks \DTcomment{Callbacks for the Lightning pipeline\: \bf 1421 lines}.
.4 dyrealloc\_callback.py \DTcomment{Run LoRA searches during training\: \bf 1403 lines}.
% .4 metrics\_callback.py \DTcomment{Extract validation results for later use\: \bf 18 lines}.
.3 pl\_model\_wrapper/ \DTcomment{Lightning wrapper classes for models\: \bf 510 lines}.
.3 projectors/ \DTcomment{Shortcut module and configuration parser\: \bf 273 lines}.
.3 tools/ \DTcomment{Auxiliary functions and plotters\: \bf 389 lines}.
% .4 checkpoint\_load.py \DTcomment{Load model checkpoint\: \bf 28 lines}.
% .4 draw\_dyrealloc\_heatmap.py \DTcomment{Plot HeteroLoRA heat maps\: \bf 76 lines}.
% .4 realloc\_lora\_rank.py \DTcomment{Generate configuration from saliency scores\: \bf 112 lines}.
% .4 trainable\_param\_printer.py \DTcomment{Print number of trainable parameters\: \bf 21 lines}.
.3 main.py \DTcomment{Loading CLI arguments and set up for pipelines\: \bf 262 lines}.
.2 tests/ \DTcomment{Unit testing\: \bf 868 lines}.
.2 experiments/ \DTcomment{Experiment directory}.
.3 ags\_output/ \DTcomment{Experiment logs}.
.3 configs/ \DTcomment{Configuration files}.
.2 python-requirement.txt \DTcomment{Python package requirement file}.
.2 README.md \DTcomment{Repository description}.
}
\caption{An overview of the project's repository. \sethlcolor{Salmon}\hl{Strongly coloured} directories contain codes slightly modified from external sources. \sethlcolor{Apricot}\hl{Lightly coloured} directories contain files heavily modified from external sources. The rest of the files have been written from scratch. Some files that do not directly contribute to the final results are omitted.}
\label{fig: repo overview}
\end{figure}


==> tables/req_analysis.tex <==
\begin{table}
    \caption{A priority and risk analysis for the main deliverables. Items marked with * are extensions.}
    \label{tab: req analysis}
    \centering
    \small
    \begin{tabular}{ccc}
    \toprule
    \textbf{Main deliverables} & \textbf{Priority} & \textbf{Risk} \\
    \midrule
    Dataset preprocessing pipeline & \textcolor{red}{High} & \textcolor{BurntOrange}{Medium} \\
    Training and testing pipeline & \textcolor{red}{High} & \textcolor{BurntOrange}{Medium} \\
    LoRA module and configuration parser & \textcolor{red}{High} & \textcolor{Green}{Low} \\
    LoRA-adapted version of OPT & \textcolor{red}{High} & \textcolor{BurntOrange}{Medium} \\
    LoRA-adapted version of RoBERTa and Gemma * & \textcolor{BurntOrange}{Medium} & \textcolor{BurntOrange}{Medium} \\
    Zero-cost saliency proxies * & \textcolor{BurntOrange}{Medium} & \textcolor{Green}{Low} \\
    ALPHA-TEST saliency proxy * & \textcolor{Green}{Low} & \textcolor{red}{High} \\
    Static HeteroLoRA  * & \textcolor{Green}{Low} & \textcolor{red}{High} \\
    Dynamic HeteroLoRA * & \textcolor{BurntOrange}{Medium} & \textcolor{red}{High} \\
    Low-rank shortcut module * & \textcolor{BurntOrange}{Medium} & \textcolor{Green}{Low} \\
    Shortcut-adapted version of OPT * & \textcolor{BurntOrange}{Medium} & \textcolor{red}{High} \\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/timetable.tex <==
\begin{table}
% \renewcommand{\arraystretch}{1.2}
\caption{Timetable and milestones}
\label{tab:timetable}
\centering
\begin{tabular}{m{0.25\linewidth}m{0.4\linewidth}m{0.3\linewidth}}
    \toprule
    \textbf{Week} & \textbf{Work} & \textbf{Milestone} \\
    \midrule
    \thead{Michaelmas weeks 0--2 \\(29/09/2023 -- 18/10/2023)} 
    & Read introductory papers. Work on proposal. 
    & Deliver a literature review to supervisors. Submit final proposal draft by 16/10/2023. \\
    \midrule
    \thead{Michaelmas weeks 3--4 \\(19/10/2023 -- 01/11/2023)} 
    & Familiarise with libraries, tools, source code, and datasets. Implement the dataset loader, LoRA, Serial Adapter, and Parallel Adapter. 
    & \\
    \midrule
    \thead{Michaelmas weeks 5--6 \\(02/11/2023 -- 15/11/2023)} 
    & Implement RoBERTa and Vicuna. Apply LoRA to these models. 
    & \\
    \midrule
    \thead{Michaelmas weeks 7--8 \\(16/11/2023 -- 29/11/2023)} 
    & Fine-tuning the adapters and complete the evaluation. Compare with previous paper results. 
    & \\
    \midrule
    \thead{Christmas vacation \\weeks 1--2 \\(30/11/2023 -- 13/12/2023)} 
    & Finish uncompleted milestones and meet the core objective. 
    & Core deliverable is done. \\
    \midrule
    \thead{Christmas vacation \\weeks 3--4 \\(14/12/2023 -- 27/12/2023)} 
    & Implement LLaMA and dataset loaders.
    & \\
    \midrule
    \thead{Christmas vacation \\weeks 5--7 \\(28/12/2023 -- 17/01/2024)} 
    & Implement Prefix Tuning and Scaled Parallel Adapter. Implement MAM Adapter. Write a draft of Introduction and Preparation of dissertation.
    & Deliver a draft of Introduction and Preparation to supervisors. \\
    \midrule
    \thead{Lent weeks 1--2 \\(18/01/2024 -- 31/01/2024)} 
    & Write Progress Report, prepare progress presentation.
    & Submit progress report by 02/02/2024. Finish slides for presentation. Rehearse for presentation. \\
    \midrule
    \thead{Lent weeks 3--4 \\(01/02/2024 -- 14/02/2024)}
    & Fine-tuning the adapters and complete the new evaluation.
    & \\
    \midrule
    \thead{Lent weeks 5--6 \\(15/02/2024 -- 28/02/2024)} 
    & Complete extensions so far. Write a draft of Method and Evaluation with results so far.
    & Deliver a draft of Method and Evaluation to supervisors and DoS. \\
    \midrule
    \thead{Lent weeks 7--8 \\(29/02/2024 -- 13/03/2024)}
    & Edit dissertation draft. Familiarise with network architecture search (NAS) and Bayesian Optimisation (BO) methods and tools.
    & \\
    \midrule
    \thead{Easter vacation weeks 1--2 \\(14/03/2024 -- 27/03/2024)}
    & Experiment on adapter shortcuts empirically. Design adapter shortcuts search space. 
    & \\
    \midrule
    \thead{Easter vacation weeks 3--4 \\(28/03/2024 -- 10/04/2024)}
    &  Search for shortcuts architecture. Complete the evaluation.
    & \\
    \midrule
    \thead{Easter vacation weeks 5--6 \\(11/04/2024 -- 24/04/2024)}
    & Complete dissertation draft with results of completed extensions.
    & Deliver dissertation draft to supervisors. \\
    \midrule
    \thead{Easter weeks 1--2 \\(25/04/2024 -- 08/05/2024)}
    & Time reserved for unexpected issues
    & Submit final dissertation and source code by 10/05/2024. \\
    \bottomrule
\end{tabular}
\end{table}

